Modified Gravity and Cosmology: An Update by the CANTATA Network

General Relativity and the $\Lambda$CDM framework are currently the standard lore and constitute the concordance paradigm. Nevertheless, long-standing open theoretical issues, as well as possible new observational ones arising from the explosive development of cosmology the last two decades, offer the motivation and lead a large amount of research to be devoted in constructing various extensions and modifications. All extended theories and scenarios are first examined under the light of theoretical consistency, and then are applied to various geometrical backgrounds, such as the cosmological and the spherical symmetric ones. Their predictions at both the background and perturbation levels, and concerning cosmology at early, intermediate and late times, are then confronted with the huge amount of observational data that astrophysics and cosmology are able to offer recently. Theories, scenarios and models that successfully and efficiently pass the above steps are classified as viable and are candidates for the description of Nature. This work is a Review of the recent developments in the fields of gravity and cosmology, presenting the state of the art, high-lighting the open problems, and outlining the directions of future research. Its realization was performed in the framework of the COST European Action ``Cosmology and Astrophysics Network for Theoretical Advances and Training Actions''.

==> 4-0_MONIZ/Moniz.tex <==
%% ****** Start of file apstemplate.tex ****** %
%%
%%
%%   This file is part of the APS files in the REVTeX 4 distribution.
%%   Version 4.1r of REVTeX, August 2010
%%
%%
%%   Copyright (c) 2001, 2009, 2010 The American Physical Society.
%%
%%   See the REVTeX 4 README file for restrictions and more information.
%%
%
% This is a template for producing manuscripts for use with REVTEX 4.0
% Copy this file to another name and then work on that file.
% That way, you always have this original template file to use.
%
% Group addresses by affiliation; use superscriptaddress for long
% author lists, or if there are many overlapping affiliations.
% For Phys. Rev. appearance, change preprint to twocolumn.
% Choose pra, prb, prc, prd, pre, prl, prstab, prstper, or rmp for journal
%  Add 'draft' option to mark overfull boxes with black boxes
%  Add 'showpacs' option to make PACS codes appear
%  Add 'showkeys' option to make keywords appear
%\documentclass[aps,prd,nofootinbib,draft]{revtex4-1}[12pt]
%\usepackage{amsmath}
%\usepackage[utf8]{inputenc}

% You should use BibTeX and apsrev.bst for references
% Choosing a journal automatically selects the correct APS
% BibTeX style file (bst file), so only uncomment the line
% below if necessary.
%\bibliographystyle{apsrev4-1}

%\begin{document}

% Use the \preprint command to place your local institutional report
% number in the upper righthand corner of the title page in preprint mode.
% Multiple \preprint commands are allowed.
% Use the 'preprintnumbers' class option to override journal defaults
% to display numbers if necessary
%\preprint{}

%Title of paper
%\title{}

% repeat the \author .. \affiliation  etc. as needed
% \email, \thanks, \homepage, \altaffiliation all apply to the current
% author. Explanatory text should go in the []'s, actual e-mail
% address or url should go in the {}'s for \email and \homepage.
% Please use the appropriate macro foreach each type of information

% \affiliation command applies to all authors since the last
% \affiliation command. The \affiliation command should follow the
% other information
% \affiliation can be followed by \email, \homepage, \thanks as well.
%\author{}
%\email[]{Your e-mail address}
%\homepage[]{Your web page}
%\thanks{}
%\altaffiliation{}
%\affiliation{}

%Collaboration name if desired (requires use of superscriptaddress
%option in \documentclass). \noaffiliation is required (may also be
%used with the \author command).
%\collaboration can be followed by \email, \homepage, \thanks as well.
%\collaboration{}
%\noaffiliation

%\date{\today}

%\begin{abstract}
% insert abstract here
%\end{abstract}

% insert suggested PACS numbers in braces on next line
%\pacs{}
% insert suggested keywords - APS authors don't need to do this
%\keywords{}

%\maketitle must follow title, authors, abstract, \pacs, and \keywords
%\maketitle

% body of paper here - Use proper section commands
% References should be done using the \cite, \ref, and \label commands
%\section{}
% Put \label in argument of \section for cross-referencing


\chapter[Outlook]{Outlook}

{\em Paulo V. Moniz}\\

%~\footnote{Departamento de F\'{i}sica, Universidade da Beira 
%Interior, Rua 
%Marqu\^{e}s d'Avila
%e Bolama, 6200 Covilh\~{a}, Portugal\\ Centro de Matem\'{a}tica e 
%Aplica\c{c}\~{o}es (CMA - UBI),
%Universidade da Beira Interior, Rua Marqu\^{e}s d'Avila
%e Bolama, 6200 Covilh\~{a}, Portugal-- 
%pmoniz@ubi.pt}}
 

 
 
 
 

It is always difficult to forecast about the future. Quoting with humility, 
Albert Einstein said that he did not worry about the future, it came too soon.  
I also heard once that the perfect counsellor would be a very, very old, really 
old person, as well as being completely, totally, absolutely mad. So, one needs 
to turn on these two features, singular madness and a sort of top intelligent 
senility. So, I don't know. Yet. 


But I will say that the main weakness of what has been Cantata in these four or 
five years, whereby investigating about dark matter and dark energy, was 
ignoring 
any explicit of string theory or equivalent. And this should be the focus of new 
actions. Bring in ‘topology above geometry’, even lines from algebraic topology, 
going more mathematical, sincerely mathematical. An action bringing mathematics 
and physics.  Besides observational data and deep analysis. I am sure that in 
our mandate for ‘action’ we had no venture in stringy or alike, by means of the 
identification of our specific aims. But, even in spite of commissars’ 
surveillance at times and in situ, we could had gone looking at such or even 
softly related new alike ventures for a time. Open mindedness, diplomacy, ‘where 
there is a will…’, wrap it up in such a way that … it passes any overzealous 
Torquemada. 


Thomas Kuhn, the historian and philosopher of science (who is not without 
controversy) said that sometimes, actually most of the times, science progresses 
within a very large set of very minor steps, which he called ‘normal science’. I 
think Cantata (possibly, surely all of us) did quite a lot of fair, honest, 
sincere, but perhaps mere normal science. It was much a very longitudinal 
research path. And the next steps (meaning action(s) emerging from Cantata) 
ought to explore (here, there, perhaps everywhere?) on the transverse. Or leap, 
with faith, into site(s). I now know this is going to sound terribly pedantic, 
but here it goes. Bringing to real life the commandments and commitments laid in 
Homer’s Odyssey, Portuguese Navigators in the 15 ~ 16th century followed the 
advice (seemed mad at the time), from good people who had the fundamental (and 
dangerous) knowledge, that to go around specific capes, unseen scientific 
evidence (given by those research ‘institutes´)  instructed they should give way 
of any navigation by the coast on sight, venture into the deep open ocean and 
pick up new fair winds that should lay ahead… just had faith. If you wait, it 
will come!  So, I said that a routing, beyond the longitudinal, trying the 
transversal, exploring whatever the perpendicular directions would had allowed, 
would (had) made a difference. 

On a complementary note, picking up an example, both allegoric as well as 
concrete (where Cantata should have had and has not properly) ventured, C. 
Kiefer, T.P Singh and a few collaborators have pioneered (through a set of 
brilliant papers2) a limited but enticing description. There is a domain where 
(quantum) gravity dominates but also another, where (a sort of) semi-classical 
is allowed and realistic. And the message was that along integral lines of the 
Hamilton-Jacobi equation, i.e., minisuperspace and some fluctuations, we have a 
fair (Cauchy wise) depiction but as we ponder the transverse, in contrast to the 
longitudinal, we know very little, if anything of reliable and is very much 
speculative; yet. Of course, the lesson is that sometimes we do need to go 
longitudinal to get a coherent road map (of the tracks and where it leads and 
connects) but sometimes the exciting new stuff to discover is beyond the 
borderline, out of beaten tracks. Think Bartolomeu, Cape of Good Hope, 1492 and 
the Alísios. That sort. Sometimes it pays to do a bit of Lewis \& Clarke. Or 
have 
a few selected ones in your team that would do it. For a while. i.e., sticking 
in going strictly geometrical, no addition of extra matter fields and couplings, 
one could still have gone into ‘lateral’, trying somewhat quite unrelated, 
explore and discover more about gravity. In this way, (no guarantees!)  we might 
have discovered more about ‘dark energy’ or whatever the hell that is or is not. 
That is the message in C Kiefer \& TP Singh seminal paper: if one wants more 
from 
(quantum) gravity, beyond the standard, you need to drop of along the 
longitudinal and probe some transverse regions. How? 
I am merely filling in words without substantive support, i.e., I am 
brainstorming. One would need to go beyond the standard exploring of standard 
geometry, consider ‘new geometry’ to unveil if gravity or whatever to gravity, 
is ‘there’. Take less classical and the usual geometries,  maybe you could 
proceed more quantum mechanical,  operational Hilbert space on states and 
unclear geometrical interpretations, topological and algebraic topological 
aspects should also be taken into consideration. All  in terms of unusual 
not-simply connected manifolds, even supermanifolds, other representations, that 
should have been pursued; in the end,  some Actions have or had nevertheless, 
then,  explored very much within normal science.

I asked to be iconoclast, so here  I am. Not sure if I am doing sense, 
conveying 
fairness but hopefully am being an Agent Provocateur, running in this field of 
gravity. 


Lines to consider (will come back to them, at the end):  causal sets, or loops 
and (spin) networks, other variables beside the metric (or not the metric at 
all), other features (e.g. torsion), have spinors intrinsically and explicit, 
get no-results or negative answers to hypothesis for gravity,  hypothesis beyond 
simple general relativity and equivalence principle, find glimpses of cracks in 
the paradigm. 
It is not that all of us in Cantata should go transverse for all the time but a 
few (selected) ones, from a few projects, ought to, for a while. And enthused to 
do so, namely within STSM or other. The element of crazy ideas, brainstorming 
the wild was never either implicit or even explicit. It was a lot of conformity. 
This however, is a fault of COST: the aim is more geopolitical, embracing, bring 
together and them managed by mediocre staff and administration, who had very few 
recognitions in terms of anyone ‘up there’ having a Nobel or Field or 
equivalent, with community recognition. The point is that you do have things as 
NSF or EPSRC or Niels Bohr institute, IAS (Princeton) and they are led or were 
led from people like old Niels. You do not have a Niels Bohr instructing COST or 
the EU commission. Surprisingly, the dictum may even come from politicians who 
have no PhD or MSc. Just the proper EU party connection. Or location, location, 
location.  It is basically mediocre and median; I admit there are and were 
politicians whom may be or had been well intentioned but majorly they were 
lacking the intellectual capacity to ask for risk taking. Now is the age of 
looking good in the Instagram with a flawless hairdo or geometrically pined tie 
around your neck and not the age of publishing audatia  papers in Annalen der 
Physik or investigating with divine commitment at Arcueil. 

And so, Cantata as others are sort of constrained to ‘be’ normal science, show a 
few (many!) papers, show a lot of countries, a lot STSM, but... the Actions are 
yet way of the output and reached peaks that ought to be. PR offices at the EU 
central ruling sites would (strongly) disagree, by means of finely chosen 
singular arguments or examples. But I do claim that this disruption hereby 
presented is worthy and healthy for progress planning. 

I hope I am allowed to point to more explicit the lines that any post-Cantata 
should (in my opinion) pursue. It is really difficult. It is like having JS 
Bach´s asking what’s next, for forthcoming centuries but where no oracle for a 
‘Ludwig van something’ is even whispered by the gods. Maybe it will be 
something 
completely different of what is below. I hope so. 

On a mathematics path, I would consider (new) algebraic approaches and 
(quantum) 
groups. Think Dirac. Genius. Got things wrong. Some, possibly. Still genius. 
Possibly something (what?) is right, when we are told to look for beauty, 
mathematically. Ditch Barbara. Keep the old man´s line: something’s a foot, that 
is the game. Look at 
non-commutative, non-associative space-times. One the one hand, keep more 
explicit about holography i.e., manipulate it, not just cite it. And I would 
take ‘causal sets’ very seriously indeed. 

I would also go beyond the beaten track of poor masters. I would explore 
(beyond) minisuperspace quantum cosmology. Beyond the boring normal science and 
take up tetrads and torsion and spinors. I.e., import the geometry ingredients 
from superstring, supergravity, namely Kahler geometry, complex manifolds, go… 
complex gravity. Twistors. Be brave. Sod off the poor pretentious masters or 
even failed ones.  Although a bit of repeated tune, there is much in Loops. 
Would say the problem is (some of) the people playing it. Maybe re-address it 
more openly, more playfully. 


Now, this may be a very dangerous ‘geodesic’. But take (quantum) chaos. The 
topic sort of collapsed and possibly due to a failure in dwelling there. 
Possibly because papers came with pain and Cost commissars wanted fast 
merchandising. But I would go this way. Related fractal structures would emerge, 
maybe breaking the space-time as we know it, maybe bringing gravity anew and 
maybe that is what dark energy may. Some nasty aspect of gravity. So, you need 
to break the icon. 

Let me return to topology and algebraic topology, more mathematics,  a better 
symbiosis between physics and mathematics. Beauty. Whatever. It does not matter 
if it is brutal (harsh modern art) or elegant pious (Romanic pre gothic) lines. 
Explore. Have fun. Play. Discover. Yes, I am being vague. I asked to be. I was 
allowed to. Thanks. 

So, I will now be self-contradictory. I think Cantata (or subsequent) needs much 
more observational physics. It should, e.g., fully embrace, espouse Euclid data. 
And from  Spider,  COMPol, Simon Observatory (CMBR).  LIGO?  Well, ok, now it 
bores. But yes, go surely for  Lisa. Use Deep Learning (Machine). 

On a self-criticism appraisal, I would recommend a far (much) better working 
groups (WG) interaction. Better meaning not just more but, yes, better. 
Efficient. Specifically, we should have had much more about and from WG2 and 
surely far more from WG3.  More people at WG2 and WG3.  Taking more data and 
sharing, challenging, telling us all about it. Provoke, challenge the dominant 
WG1, bringing glimpses  of glitches and cracks on data,  that would shake the 
conformity and box comfort. Aka, normal science.  

And as piéce de resistance, I would welcome being really open and allowed to be 
challenged, to justify, to explain, to convince, to be unmounted and have 
difficulty fitting in. It woks for some people. Concretely, I would say that 
going Science \& Religion may open up ontological questions and force (somehow) 
to re-group and re-stress and re-focus on very concise and precise theoretical 
physics conundrums. Some people do an evening jog, other walk long hours, others 
(or a part of those former sets) go somewhere to listen. And they are really, 
totally, absolutely, completely, covariant and invariant agnostic. But they like 
challenges. 






 


